How Gender and Birth Order Affect Educational attainment Inequality within-Families: Evidence from Benin

This paper examines how gender, birth order, and innate ability shape within-household disparities in children's educational attainment in developing countries. Using data from Benin, I find that in households with non-educated parents, gender and birth order drive over two-thirds of the average educational attainment disparities among adult children, while their influence decreases to one-third in households with college-educated parents. Furthermore, average inequality, measured by the range of children's educational attainment is twice as high among non-educated parents compared to college-educated parents. I propose and estimate a structural model of educational attainment choices within-family. Using the model, I show that the absence of gender and birth order effects does not lead to a significant reduction in the average within-family disparities in children's educational attainment. Additionally, in theory, ensuring that every child has at least one year of education lowers average within-family educational inequality. Yet, even in this scenario, daughters tend to receive less education than sons, and practical efforts to achieve universal entry are less effective than the theoretical model.

==> Tables/bias_effect.tex <==

{
\scalebox{0.8}{
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{2}{c}{Disadvantages effect on inequality} & \multicolumn{2}{c}{Extra ability needed to compensate for disadvantage effects} \\ 
\\[-1.8ex] & $q_T = 12$ & $q_T = 20$ & $q_T = 12$ & $q_T = 20$ \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 \\[-1.8ex] & \multicolumn{4}{c}{} \\
 Gender disadvantage & 2.36 (43.7\%) & 2.87 (52\%) & 14\% &8.7\%  \\ 
   & &  &  &  \\ 
 Birth order disadvantage  & 3.04(56.3\%) &2.65 (48\%) & 13\% &8.3\% \\ 
  & &  &  &  \\ 
 Both & 5.4 &5.52 & 27\%  & 17\% \\ 
 \\[-1.8ex] & \multicolumn{4}{c}{} \\
\hline 
\hline \\[-1.8ex] 

\end{tabular} 
}
}

==> Tables/counterfactual.tex <==
{
\scalebox{0.8}{
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 %& \multicolumn{4}{c}{\textit{Dependent variable}} \\ 
%\cline{2-5} 
\\[-1.8ex] & \multicolumn{2}{c}{Proportion of explained inequality} \\ 
%\\[-1.8ex] & \multicolumn{2}{c}{\textit{probit}} & \multicolumn{2}{c}{\textit{OLS}} \\ 
\\[-1.8ex] & $q_T = 12$ & $q_T = 20$ \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
\\[-1.8ex] \multicolumn{3}{c}{Same gender households} \\
 Birth order disadvantage & 64.7\% & 43.9\% \\ 
  & &    \\
Unexplained & 35.3\% & 56.1\% \\ 
\hline 
\\[-1.8ex] \multicolumn{3}{c}{Both gender households} \\
 Birth order disadvantage & 48.8\% & 35.66\% \\ 
  & &    \\
 Gender disadvantage & 37.9\% & 38.63\% \\ 
   & &  \\ 
 Both & 86.7\% &74.29\%  \\ 
  & &   \\ 
 Unexplained & 13.3\% & 25.7\% \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 
}
}

==> Tables/data_model_mom.tex <==
{
\scalebox{0.8}{
\begin{tabular}{@{\extracolsep{5pt}}lllll} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 &  & \multicolumn{1}{c}{Data Moments} & \multicolumn{1}{c}{Model moments}  & Difference  \\ 
\hline \\[-1.8ex] 

 & $\Bar{Y}_d^d - \Bar{Y}_d^b$ & 1.7028 & 1.7169& -0.0141\\ 
Non-educated parents & $\Bar{Y}_{sb}^d - \Bar{Y}_{fb}^d$ & 0.2754 & 0.4502 & -0.1748\\ 
 & $\Bar{Y}_{sb}^s - \Bar{Y}_{fb}^s$ & 0.3682 & 0.1616 & 0.2066\\

 & Proportion of educated firstborn & 0.3642 & 0.3678 & 0.0036\\

 & Proportion of educated firstborn daughters & 0.1116 & 0.1156 & 0.004\\

 & Proportion of educated second born daughters & 0.3177 & 0.3177 & 0\\
\hline \\[-1.8ex] 

&  $\Bar{Y}_d^d - \Bar{Y}_d^b$ & 1.56 & 1.55 & 0.01 \\ 
College educated parents& $\Bar{Y}_{sb}^d - \Bar{Y}_{fb}^d$ &  2.61 & 2.76 & -0.15\\ 
 & $\Bar{Y}_{sb}^s - \Bar{Y}_{fb}^s$  & 2.47 & 2.88 & -0.41 \\

 & Proportion of educated firstborn & &  & \\
 
 & Proportion of educated firstborn daughters &  &  & \\

 & Proportion of educated second born daughters &  &  & \\
\hline \\[-1.8ex] 
\end{tabular}}
}

==> Tables/data_model_non_targeted_moments.tex <==
{
\scalebox{0.8}{
\begin{tabular}{@{\extracolsep{5pt}}lllll} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 &  & \multicolumn{1}{c}{Data Moments} & \multicolumn{1}{c}{Model moments}  & Difference  \\ 
\hline \\[-1.8ex] 

 & Average inequality & 5.87 & 5.97 & -0.1\\
 \addlinespace
& Average inequality (only daughters households) &  5.29 & 5.46 & -0.17\\
\addlinespace
 & Average inequality (only sons households)  & 5.71 & 5.87 & -0.16\\
 \addlinespace

 & Average inequality (both gender households) & 6.29 & 6.29 & 0\\
\addlinespace
 & Average inequality ($\Bar{q} < 6$) & 5.05 & 5.04 & 0.01\\
\addlinespace
Non-educated parents  & Average inequality ($ 6 \leq \Bar{q} < 10$) & 8.46 & 7.56 & 0.9\\
 \addlinespace
& Average inequality ($ 10 \leq \Bar{q} < 13$) &5.27  & 5.34 & -0.07\\
\addlinespace
& Average inequality ($ \Bar{q} \geq 13$) & 2.1 & 5.62 & -3.52\\
\addlinespace
& Average inequality (intensive margin) & 3.59 & 3.77 & -0.18 \\
\addlinespace
& Standard deviation of firstborn's education & 5.55 & 5.5 &  \\
\addlinespace
& Standard deviation of second born education & 5.19 & 5.29 &  \\
\hline \\[-1.8ex] 

 & Average inequality &  & & \\ 
 \addlinespace
 & Average inequality (only daughters households) &  & & \\ 
 \addlinespace
 & Average inequality (only sons households) &  &  & \\
\addlinespace
 & Average inequality (both gender households) &  &  & \\
\addlinespace
 & Average inequality ($\Bar{q} < 6$) &  &  & \\
\addlinespace
College educated parents & Average inequality ($ 6 \leq \Bar{q} < 10$) &  &  & \\
 \addlinespace
& Average inequality ($ 10 \leq \Bar{q} < 13$) &  &  & \\
\addlinespace
& Average inequality ($ \Bar{q} \geq 13$) &  &  & \\
\addlinespace
& Average inequality (intensive margin) &  &  & \\
\addlinespace
& Standard deviation of firstborn's education &  &  &  \\
\addlinespace
& Standard deviation of second born education &  &  &  \\
\hline \\[-1.8ex] 
\end{tabular}}
}

==> Tables/observed_unobs_c.tex <==
{
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{Observed} & \multicolumn{1}{c}{Unobserved}   \\ 
\hline \\[-1.8ex] 
& \multicolumn{2}{c}{Average years of education} \\

Male & 5.35 & 4.66 \\ 
Female & 4.73 & 2.03  \\ 
Difference & 0.62& 2.63\\
\hline \\[-1.8ex] 

& \multicolumn{2}{c}{Proportion of married} \\
Male & 0.37 & 0.84 \\ 
Female & 0.38 & 0.88  \\ 
Difference & 0.01& -0.04\\
\hline \\[-1.8ex] 
\end{tabular} 
}

==> Tables/q_T_reg.tex <==
{
\begin{tabular}{l c}
\hline
 & $q_T$ \\
\hline
(Intercept)   & $16.36^{*}$       \\
          %    & $ [15.43; 17.29]$ \\
High school graduate hh   & $9.98^{*}$        \\
          %    & $ [ 9.47; 10.49]$ \\
Number of children = 2           & $-6.83^{*}$       \\
         %     & $ [-7.79; -5.87]$ \\
Number of children = 3           & $-4.33^{*}$       \\
        %      & $ [-5.29; -3.36]$ \\
Number of children = 4           & $-2.80^{*}$       \\
         %     & $ [-3.77; -1.82]$ \\
Number of children = 5           & $-1.78^{*}$       \\
       %       & $ [-2.77; -0.79]$ \\
Number of children = 6           & $-1.49^{*}$       \\
     %         & $ [-2.50; -0.48]$ \\
Number of children = 7           & $-0.95$           \\
 %             & $ [-2.01;  0.11]$ \\
Number of children = 8           & $-0.36$           \\
   %           & $ [-1.44;  0.71]$ \\
Number of children =9           & $1.19$            \\
  %            & $ [-0.06;  2.44]$ \\
Urban         & $2.73^{*}$        \\
    %          & $ [ 2.43;  3.02]$ \\
Christian     & $3.27^{*}$        \\
    %          & $ [ 3.00;  3.54]$ \\
High hwi     & $2.16^{*}$        \\
       %       & $ [ 1.87;  2.45]$ \\
Head of household is farmer & $-3.43^{*}$       \\
         %     & $ [-3.64; -3.21]$ \\
\hline
R$^2$         & $0.20$            \\
Adj. R$^2$    & $0.20$            \\
Num. obs.     & $29713$           \\
RMSE          & $11.14$           \\
\hline
\multicolumn{2}{l}{\scriptsize{$^*$ 0 outside the confidence interval.}}
\end{tabular}
}

==> Tables/quantity_quality.tex <==
{
\begin{tabular}{l c c c c c c}
\hline
& \multicolumn{2}{c} {1998-2013} & \multicolumn{2}{c} {1970-1998} & \multicolumn{2}{c} {1960-1970}\\
 & OLS & IV & OLS & IV & OLS & IV \\
\hline
(Intercept)         & $0.74^{*}$        & $0.71^{***}$  & $0.44^{*}$        & $0.46^{***}$  & $0.16^{*}$        & $0.62^{*}$    \\
                    & $ [ 0.74;  0.75]$ & $(0.01)$      & $ [ 0.43;  0.44]$ & $(0.02)$      & $ [ 0.12;  0.19]$ & $(0.26)$      \\
Family size:Urban & $-0.01^{*}$       & $-0.01^{***}$ & $-0.00^{*}$       & $-0.00$       & $0.00$            & $0.01$        \\
                    & $ [-0.01; -0.01]$ & $(0.00)$      & $ [-0.00; -0.00]$ & $(0.01)$      & $ [-0.01;  0.01]$ & $(0.06)$      \\
Family size:Rural & $-0.02^{*}$       & $-0.02^{***}$ & $-0.00^{*}$       & $-0.01^{*}$   & $0.00$            & $-0.16$       \\
                    & $ [-0.03; -0.02]$ & $(0.00)$      & $ [-0.00; -0.00]$ & $(0.00)$      & $ [-0.00;  0.01]$ & $(0.10)$      \\
Education of hh           & $0.02^{*}$        & $0.02^{***}$  & $0.03^{*}$        & $0.03^{***}$  & $0.05^{*}$        & $0.05^{***}$  \\
                    & $ [ 0.02;  0.02]$ & $(0.00)$      & $ [ 0.03;  0.03]$ & $(0.00)$      & $ [ 0.05;  0.06]$ & $(0.00)$      \\
Female hh         & $0.09^{*}$        & $0.10^{***}$  & $0.11^{*}$        & $0.11^{***}$  & $0.15^{*}$        & $0.03$        \\
                    & $ [ 0.09;  0.09]$ & $(0.00)$      & $ [ 0.11;  0.12]$ & $(0.01)$      & $ [ 0.13;  0.17]$ & $(0.09)$      \\
HWI                 & $0.04^{*}$        & $0.04^{***}$  & $0.06^{*}$        & $0.06^{***}$  & $0.07^{*}$        & $0.07^{***}$  \\
                    & $ [ 0.04;  0.04]$ & $(0.00)$      & $ [ 0.06;  0.06]$ & $(0.00)$      & $ [ 0.06;  0.08]$ & $(0.01)$      \\
Urban               & $0.02^{*}$        & $0.04^{***}$  & $0.13^{*}$        & $0.11^{***}$  & $0.16^{*}$        & $-0.36$       \\
                    & $ [ 0.02;  0.02]$ & $(0.01)$      & $ [ 0.12;  0.13]$ & $(0.03)$      & $ [ 0.12;  0.19]$ & $(0.30)$      \\
Birth order        & $0.02^{*}$        & $0.01^{***}$  & $0.01^{*}$        & $0.02^{***}$  & $0.01$            & $0.12$        \\
                    & $ [ 0.01;  0.02]$ & $(0.00)$      & $ [ 0.01;  0.01]$ & $(0.00)$      & $ [-0.01;  0.03]$ & $(0.08)$      \\
Female              & $-0.04^{*}$       & $-0.04^{***}$ & $-0.08^{*}$       & $-0.08^{***}$ & $-0.12^{*}$       & $-0.14^{***}$ \\
                    & $ [-0.04; -0.04]$ & $(0.00)$      & $ [-0.09; -0.08]$ & $(0.00)$      & $ [-0.14; -0.10]$ & $(0.02)$      \\
\hline
R$^2$               & $0.14$            & $0.14$        & $0.21$            & $0.21$        & $0.27$            & $-0.05$       \\
Adj. R$^2$          & $0.14$            & $0.14$        & $0.21$            & $0.21$        & $0.27$            & $-0.05$       \\
Num. obs.           & $2069182$         & $2069182$     & $403850$          & $403850$      & $6461$            & $6461$        \\
RMSE                & $0.40$            &             & $0.43$            &             & $0.40$            &             \\
\hline
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$ (or Null hypothesis value outside the confidence interval).}}
\end{tabular}
}

==> Tables/reg_bias_effect.tex <==
{
\scalebox{0.93}{
\begin{tabular}{l c c c c}
\hline
& $q_T = 12$ & $q_T = 20$ &  $q_T = 12$ & $q_T = 20$ \\
 & (1) & (2) & (3) & (4) \\
\hline
(Intercept)          & $0.51$            & $-0.47$           & $-1.19$           & $-2.10$           \\
%                     & $ [-0.55;  1.58]$ & $ [-1.63;  0.69]$ & $ [-3.47;  1.10]$ & $ [-4.80;  0.59]$ \\
female\_fb           & $-5.46^{*}$       & $-4.82^{*}$       & $-5.23^{*}$       & $-4.99^{*}$       \\
%                     & $ [-6.93; -4.00]$ & $ [-6.59; -3.04]$ & $ [-6.74; -3.73]$ & $ [-6.81; -3.16]$ \\
hh educ = Primary &                   &                   & $0.68$            & $2.36^{*}$        \\
%                     &                   &                   & $ [-0.99;  2.35]$ & $ [ 0.32;  4.41]$ \\
hh educ = Junior HS &                   &                   & $2.16$            & $4.12^{*}$        \\
%                     &                   &                   & $ [-0.28;  4.60]$ & $ [ 1.60;  6.63]$ \\
hh educ = Senior HS &                   &                   & $4.41^{*}$        & $1.09$            \\
%                     &                   &                   & $ [ 0.29;  8.53]$ & $ [-1.31;  3.50]$ \\
hh educ = College &                   &                   & $2.90$            & $-0.35$           \\
%                     &                   &                   & $ [-0.16;  5.96]$ & $ [-5.44;  4.75]$ \\
HWI                  &                   &                   & $0.83^{*}$        & $-0.45$           \\
%                     &                   &                   & $ [ 0.10;  1.56]$ & $ [-1.45;  0.55]$ \\
Urban                &                   &                   & $-0.74$           & $2.14$            \\
%                     &                   &                   & $ [-2.47;  0.99]$ & $ [-0.00;  4.28]$ \\
Christian            &                   &                   & $1.73$            & $-1.21$           \\
%                     &                   &                   & $ [-0.25;  3.72]$ & $ [-3.33;  0.92]$ \\
\hline
R$^2$                & $0.16$            & $0.10$            & $0.22$            & $0.15$            \\
Adj. R$^2$           & $0.15$            & $0.09$            & $0.19$            & $0.12$            \\
Num. obs.            & $285$             & $275$             & $285$             & $275$             \\
RMSE                 & $6.28$            & $7.45$            & $6.15$            & $7.33$            \\
\hline
\multicolumn{5}{l}{\scriptsize{$^*$ Null hypothesis value outside the confidence interval.}}
\end{tabular}}
}



==> Tables/summary_stats.tex <==
{
\scalebox{0.8}{
\begin{tabular}{lccccc} 
 \hline

 & All & Only daughters & Only sons &Both gender: Female first born & Both gender: Male first born\\ [0.5ex] 
 \hline\hline
  & \multicolumn{5}{c}{} \\
  & \multicolumn{5}{c}{$q_T = 12$} \\ 
    & \multicolumn{5}{c}{$s = 5, S_d^d = 610, S_d^b = 1410, S_s^s = 1435$} \\ 
   & \multicolumn{5}{c}{} \\
 Number of observations & 740 & 126  & 308 &161 &156  \\ [1ex]

Average range (Data) & 4.94 & 3.8 & 5.07 &6.23 & 4.04  \\ [1ex]
 & & \multicolumn{2}{c}{Same gender: 4.70} && \\

Average range (Model) & 3.52 & 3.25 & 3.27 &5.04 & 2.38  \\ [1ex]
 & & \multicolumn{2}{c}{Same gender: 3.26} && \\
 & \multicolumn{5}{c}{\textcolor{blue}{$\Hat{\theta}_{(2, 12)} = (0.0625, 0.027)$}} \\
  & \multicolumn{5}{c}{\textcolor{blue}{$se = (0.0094, 0.0028)$}} \\
%  & \multicolumn{5}{c}{} \\
 \hline
 \hline
 & \multicolumn{5}{c}{} \\
 & \multicolumn{5}{c}{$q_T = 20$} \\
     & \multicolumn{5}{c}{$s = 5, S_d^d = 625, S_d^b = 1365, S_s^s = 1280$} \\ 
  & \multicolumn{5}{c}{} \\
  Number of observations & 654 & 125  & 256 &138 &135  \\ [1ex]

Average range (Data) & 6.09 & 5.87 & 6.12 & 7.43 & 4.86  \\ [1ex]
 & & \multicolumn{2}{c}{Same gender: 6.04}&& \\
 Average range (Model) & 4.71 & 4.60 & 4.54 & 5.99 & 3.84  \\ [1ex]
 & & \multicolumn{2}{c}{Same gender: 4.56}&& \\
 & \multicolumn{5}{c}{} \\
 & \multicolumn{5}{c}{\textcolor{red}{$\Hat{\theta}_{(2, 20)} = (0.0351, 0.0106)$}} \\
  & \multicolumn{5}{c}{\textcolor{red}{$se = (0.0069, 0.0015)$}} \\
%  & \multicolumn{5}{c}{} \\
 \hline
 \hline
\end{tabular}}
}



==> Tables/table2.tex <==
{
\begin{tabular}{@{\extracolsep{5pt}}lc} 

\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & Within household standard  \\ 
\\[-1.8ex] &  deviation of education attainment \\ 
\hline \\[-1.8ex] 
 High school graduate hh & $-$0.630$^{***}$ \\ 
  & (0.063) \\ 

 Number of children & 0.045$^{***}$ \\ 
  & (0.009) \\ 

 HWI & $-$0.125$^{***}$ \\ 
  & (0.018) \\ 

Rrural & $-$0.243$^{***}$ \\ 
  & (0.050) \\ 

Average Years of education & $-$0.093$^{***}$ \\ 
  & (0.004) \\ 
  
 Christian & $-$0.268$^{***}$ \\ 
  & (0.035) \\ 

 Number of Spouse & 0.124$^{***}$ \\ 
  & (0.034) \\ 

 Both gender & 0.211$^{***}$ \\ 
  & (0.042) \\ 

 Constant & 4.424$^{***}$ \\ 
  & (0.063) \\ 
\hline \\[-1.8ex] 
Observations & 29,713 \\ 
R$^{2}$ & 0.064 \\ 
Adjusted R$^{2}$ & 0.063 \\ 
Residual Std. Error & 2.784 (df = 29703) \\ 
F Statistic & 224.741$^{***}$ (df = 9; 29703) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
}

==> Tables/table3.tex <==
{
\begin{tabular}{p{2cm} p{2cm} p{2cm}} 
 \hline
Test & p-value (CT) & p-value (UT) \\ [0.5ex] 
 \hline\hline
RCIT & 0.27 & 0  \\ [1ex]
 \hline
RCoT& 0.47 & 0\\[1ex]
 \hline
GCM & 0.79 & 0\\[1ex]
 \hline
 \hline
\end{tabular}
}
